Speeding up MadGraph5_aMC@NLO

In this paper we will describe two new optimisations implemented in MadGraph5_aMC@NLO, both of which are designed to speed-up the computation of leading-order processes (for any model). First we implement a new method to evaluate the squared matrix element, dubbed helicity recycling, which results in factor of two speed-up. Second, we have modified the multi-channel handling of the phase-space integrator providing tremendous speed-up for VBF-like processes (up to thousands times faster).

==> input/born.tex <==
%\feynmandiagram[horizontal=a to b] {
%	i1 [particle=\(e^{-}\)] -- [fermion, momentum'={[arrow shorten=0.25]\(p_1\)}] a -- [fermion, reversed momentum'={[arrow shorten=0.25]\(p_2\)}] i2 [particle=\(e^{+}\)],
%	a -- [photon,edge label=\(\gamma\)] b,
%	f1 [particle=\(\mu^{+}\)] -- [fermion, reversed momentum'={[arrow shorten=0.25]\(p_4\)}] b,
%	b -- [fermion,momentum'={[arrow shorten=0.25]\(p_3\)}] f2 [particle=\(\mu^{-}\)],
%};
\feynmandiagram[horizontal=a to b] {
    i1 [particle=\(e^{+}\)] -- [anti fermion, momentum'={[arrow shorten=0.25]\(p_2\)}] a -- [anti fermion, reversed momentum'={[arrow shorten=0.25]\(p_1\)}] i2 [particle=\(e^{-}\)],
%	a -- [photon,edge label=\(\gamma\)] b,
	a -- [photon,edge label=\(\gamma\)] b,
	f1 [particle=\(\mu^{-}\)] -- [anti fermion, reversed momentum'={[arrow shorten=0.25]\(p_3\)}] b,
	b -- [anti fermion,momentum'={[arrow shorten=0.25]\(p_4\)}] f2 [particle=\(\mu^{+}\)],
};
